Continuous Execution of High-Level Collaborative Tasks for Heterogeneous Robot Teams

We propose a control synthesis framework for a heterogeneous multi-robot system to satisfy collaborative tasks, where actions may take varying duration of time to complete. We encode tasks using the discrete logic LTL^\psi, which uses the concept of bindings to interleave robot actions and express information about relationship between specific task requirements and robot assignments. We present a synthesis approach to automatically generate a teaming assignment and corresponding discrete behavior that is correct-by-construction for continuous execution, while also implementing synchronization policies to ensure collaborative portions of the task are satisfied. We demonstrate our approach on a physical multi-robot system.

==> algs/update_trace_old.tex <==
For each transition $(z, \sigma, z'), z \neq z'$ and possible teaming assignment $R$, each robot

\begin{enumerate}
    \item synthesizes discrete behavior $\sigma^{z,z'}_j$, $q_{j,wait} = \sigma^{z,z'}_j[end-1], q_{j,sync} = \sigma^{z,z'}_j[end]$
    \item check if intermediate traces should be checked ($|\mathfrak{I}(s, s')| > 1$)
    \item If yes
    \begin{enumerate}
        \item each possible intermediate trace is generated by checking every ordering of robots for every step in trace where at least one robot changes AP state (TODO)
        \item check that each step in updated team trace does not violate 
    \end{enumerate}
\end{enumerate}




\begin{equation}
  \mathfrak{I}(s, s') =
    \begin{cases}
      True & \text{if $L(s) \cap AP_{non-inst} \neq L(s') \cap AP_{non-inst}$}\\
      False & \text{otherwise}\\
    \end{cases}       
\end{equation}

\begin{algorithm}[h]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Initialization}{Initialization}{}{}
\Input{$(z,\sigma, z')$, $\delta_{self}$, $A = \{A_1,A_2, ...,A_n\}, R = \{r_1,r_2, ...,r_n\}$, $\mathcal{G} = \{\mathcal{G}_1, \mathcal{G}_2, ..., \mathcal{G}_n \}$}
\Output{$\sigma^{z, z'}$}

\For{$A_j \in A$}{
    $b_j= \textsc{find\_behavior}(\mathcal{G}_j, r_j, (z,\sigma, z'), \delta_{self})$ \\
}
$\sigma^{z, z'} = b_1b_2...b_n$, \ $\hat{b}_1\hat{b}_2...\hat{b}_n = b_1(1)b_2(1)...b_n(1)$ \\
% $\ell = length(b_1)$

\For{$i \in \{1, ..., length(b_1)-1 \}$}{
    \tcp{only look agents that have non-inst transitions within sub-trace}
    $A' = \{A_j \in A \ | \ \mathfrak{I}(b_j(i), b_j(i+1)) = True\}$ \\
    \If{$|A'| \leq 1$}{
    % $\hat{b}_1\hat{b}_2...\hat{b}_n = b_1b_2...b_n$ \\
    $\hat{b}_j = \hat{b}_j + b_j(i) \ \ \forall j = \{1,2,...,n\}$ \\
    \textbf{continue}
    }
    $ordering = \textsc{permuations($A'$)}$ \\
    $violation = False$ \\
    \For{$order \in ordering$}{
        \tcp{generate all intermediate traces}
        $w=0$ \\
        \For{$A_j \in order$}{
        $q = b_j(i), q'= b_j(i+1)$ \\
        $b_j^{int} = q*(w+1) + q'*(length(order)-w)$ \\
        $w = w + 1$ \\
        }
        $violation = \textsc{check\_intermediate\_trace}(\sigma, b_1^{int}b_2^{int}...)$ \\
        \tcp{found valid intermediate trace}
        \If{not $violation$}{
        \For{$A_j \in A$}{
            \If{$A_j \in A'$}{
            % $\hat{b}_j(i:i+1) = b_j^{int}$
            $\hat{b}_j = \hat{b}_j + b_j^{int}(2:end)$
            }
            \tcp{agents that do not have non-inst actions, just update length}
            \Else{
            % $\hat{b}_j(i) = b_j(i)*length(order)$
            $\hat{b}_j = \hat{b}_j + b_j(i)*(length(order)-1) + b_j(i+1)$
            }
        }
        \textbf{break}
        % \For{$b_j^{z, z'} \in \sigma^{z, z'}$}{
        %     $b_j^{z, z'}(i:i+1) = b_j^{int}$ \\
        %     \textbf{break}
        %     }
        }
    }

    \tcp{if all possible intermediate traces violate}
    \If{violation}{
    \Return
    }
    
}
% $\sigma_{int}^{z, z'} = b_1^{int}b_2^{int}...b_n^{int}$ \\
% \For{$b_j^{z, z'} \in \sigma^{z, z'}$}{
% $b_j^{z, z'}(i:i+1) = b_j^{int}$
% }
\Return $\sigma_{int}^{z, z'} = \hat{b}_1\hat{b}_2...\hat{b}_n $
   
\caption{Update Trace}
\end{algorithm}
